On Demographic Group Fairness Guarantees in Deep Learning

We present a theoretical framework analyzing the relationship between data distributions and fairness guarantees in equitable deep learning. We establish novel bounds that account for distribution heterogeneity across demographic groups, deriving fairness error and convergence rate bounds that characterize how distributional differences affect the fairness-accuracy trade-off. Extensive experiments across diverse modalities, including FairVision, CheXpert, HAM10000, FairFace, ACS Income, and CivilComments-WILDS, validate our theoretical findings, demonstrating that feature distribution differences across demographic groups significantly impact model fairness, with disparities particularly pronounced in racial categories. Motivated by these insights, we propose Fairness-Aware Regularization (FAR), a practical training objective that minimizes inter-group discrepancies in feature centroids and covariances. FAR consistently improves overall AUC, ES-AUC, and subgroup performance across all datasets. Our work advances the theoretical understanding of fairness in AI systems and provides a foundation for developing more equitable algorithms. The code for analysis is publicly available at https://github.com/Harvard-AI-and-Robotics-Lab/FairnessGuarantee.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> sec/backup_content.tex <==
\begin{theorem}[Fairness Error Bound]
Let $\mathcal{F}$ be a class of functions mapping from the input space $\mathcal{X}$ to the output space $\mathcal{Y}$, and let $\ell: \mathcal{Y} \times \mathcal{Y} \to [0, 1]$ be a loss function. Assume that for each demographic group $a_i$, the data distribution $\mathcal{D}_{a_i}$ satisfies the following assumptions:

The input space $\mathcal{X}$ is a compact subset of $\mathbb{R}^d$.
The function class $\mathcal{F}$ is Lipschitz continuous with respect to the input $x$, i.e., there exists a constant $L > 0$ such that for all $f \in \mathcal{F}$ and $x, x' \in \mathcal{X}$, $|f(x) - f(x')| \leq L |x - x'|$.
Let $S_{a_i} = {(x_1^{a_i}, y_1^{a_i}), \ldots, (x_n^{a_i}, y_n^{a_i})}$ be a sample of size $n$ drawn i.i.d. from $\mathcal{D}_{a_i}$ for each demographic group $a_i$. Then, with probability at least $1 - \delta$, for all $f \in \mathcal{F}$ and all pairs of demographic groups $a_i, a_j$, the following holds:

\begin{align*}
&\left| \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x), y)] \right| \ \\
 \leq& \left| \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_i}), y_k^{a_i}) - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_j}), y_k^{a_j}) \right| + 2\mathcal{R}_n(\ell \circ \mathcal{F}) + \sqrt{\frac{2\ln(4k/\delta)}{n}}
\end{align*}

where $\mathcal{R}_n(\ell \circ \mathcal{F})$ is the Rademacher complexity of the composed function class $\ell \circ \mathcal{F} = {\ell(f(\cdot), \cdot) : f \in \mathcal{F}}$.
\end{theorem}

\begin{proof}
For a fixed pair of demographic groups $a_i, a_j$, define the random variable
\begin{align*}
Z_{ij} = \mathbb{E}{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x), y)] - \mathbb{E}{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x), y)]
\end{align*}

and its empirical counterpart
\begin{align*}
\hat{Z}{ij} = \frac{1}{n} \sum{k=1}^n \ell(f(x_k^{a_i}), y_k^{a_i}) - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_j}), y_k^{a_j})
\end{align*}

We can bound the difference between $Z_{ij}$ and $\hat{Z}_{ij}$ using the Rademacher complexity and Hoeffding's inequality.

\begin{lemma}[Rademacher Complexity Bound]
Let $\mathcal{G}$ be a class of functions mapping from a space $\mathcal{Z}$ to $[0, 1]$. Then, with probability at least $1 - \delta/2$, for all $g \in \mathcal{G}$, the following holds:
\begin{align*}
\mathbb{E}[g(Z)] \leq \frac{1}{n} \sum_{k=1}^n g(Z_k) + 2\mathcal{R}_n(\mathcal{G}) + \sqrt{\frac{\ln(2/\delta)}{2n}}
\end{align*}
where $Z_1, \ldots, Z_n$ are i.i.d. samples from $\mathcal{Z}$, and $\mathcal{R}_n(\mathcal{G})$ is the Rademacher complexity of $\mathcal{G}$.
\end{lemma}

Applying the Rademacher complexity bound to the function class $\ell \circ \mathcal{F}$ and the data distributions $\mathcal{D}{a_i}$ and $\mathcal{D}{a_j}$ separately, we have with probability at least $1 - \delta/2$, for all $f \in \mathcal{F}$:
\begin{align*}
&\mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x), y)] \\
\leq& \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_i}), y_k^{a_i}) + 2\mathcal{R}n(\ell \circ \mathcal{F}) + \sqrt{\frac{\ln(4/\delta)}{2n}} \
\mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x), y)] \\
\geq& \frac{1}{n} \sum{k=1}^n \ell(f(x_k^{a_j}), y_k^{a_j}) - 2\mathcal{R}_n(\ell \circ \mathcal{F}) - \sqrt{\frac{\ln(4/\delta)}{2n}}
\end{align*}

Combining these inequalities and applying the union bound over all $k(k-1)/2$ pairs of demographic groups, we obtain the desired result with probability at least $1 - \delta$.
\end{proof}

\begin{theorem}[Fairness Error Bound]
Let $\mathcal{F}$ be a class of functions mapping from the input space $\mathcal{X}$ to the output space $\mathcal{Y}$, and let $\ell: \mathcal{Y} \times \mathcal{Y} \to [0, M]$ be a bounded loss function. Assume that for each demographic group $a_i \in \mathcal{A}$, the data distribution $\mathcal{D}_{a_i}$ satisfies the following assumptions:

The input space $\mathcal{X}$ is a measurable space.
The function class $\mathcal{F}$ has a finite Vapnik-Chervonenkis (VC) dimension $d < \infty$.
Let $S_{a_i} = {(x_1^{a_i}, y_1^{a_i}), \ldots, (x_n^{a_i}, y_n^{a_i})}$ be a sample of size $n$ drawn i.i.d. from $\mathcal{D}_{a_i}$ for each demographic group $a_i$. Then, with probability at least $1 - \delta$, for all $f \in \mathcal{F}$ and all pairs of demographic groups $a_i, a_j \in \mathcal{A}$, the following holds:

\begin{align*}
&\left| \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x), y)] \right| \
\quad \\
\leq& \left| \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_i}), y_k^{a_i}) - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_j}), y_k^{a_j}) \right| + 2M\sqrt{\frac{2d\log(2en/d) + \log(8|\mathcal{A}|^2/\delta)}{n}}
\end{align*}
where $|\mathcal{A}|$ is the cardinality of the demographic attribute set $\mathcal{A}$.
\end{theorem}

\begin{proof}
For a fixed pair of demographic groups $a_i, a_j \in \mathcal{A}$, define the random variable
\begin{align*}
Z_{ij} = \mathbb{E}{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x), y)] - \mathbb{E}{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x), y)]
\end{align*}

and its empirical counterpart
\begin{align*}
\hat{Z}{ij} = \frac{1}{n} \sum{k=1}^n \ell(f(x_k^{a_i}), y_k^{a_i}) - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_j}), y_k^{a_j})
\end{align*}

We can bound the difference between $Z_{ij}$ and $\hat{Z}_{ij}$ using the Vapnik-Chervonenkis (VC) inequality.

\begin{lemma}[Vapnik-Chervonenkis Inequality]
Let $\mathcal{G}$ be a class of functions mapping from a measurable space $\mathcal{Z}$ to $[0, M]$ with VC dimension $d < \infty$. Then, with probability at least $1 - \delta/2$, for all $g \in \mathcal{G}$, the following holds:
\begin{align*}
\left| \mathbb{E}[g(Z)] - \frac{1}{n} \sum_{k=1}^n g(Z_k) \right| \leq M\sqrt{\frac{2d\log(2en/d) + \log(4/\delta)}{n}}
\end{align*}
where $Z_1, \ldots, Z_n$ are i.i.d. samples from $\mathcal{Z}$.
\end{lemma}

Applying the VC inequality to the function class $\ell \circ \mathcal{F}$ and the data distributions $\mathcal{D}{a_i}$ and $\mathcal{D}{a_j}$ separately, we have with probability at least $1 - \delta/2$, for all $f \in \mathcal{F}$:
\begin{align*}
&\left| \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x), y)] - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_i}), y_k^{a_i}) \right| \\
\leq &M\sqrt{\frac{2d\log(2en/d) + \log(8/\delta)}{n}} \
\left| \mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x), y)] - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_j}), y_k^{a_j}) \right| \\
\leq& M\sqrt{\frac{2d\log(2en/d) + \log(8/\delta)}{n}}
\end{align*}

Combining these inequalities using the triangle inequality and applying the union bound over all $|\mathcal{A}|(|\mathcal{A}|-1)/2$ pairs of demographic groups, we obtain the desired result with probability at least $1 - \delta$.
\end{proof}

\subsection{Error Bound}

To provide an error bound for the fairness problem using optimal transport, we will assume that the data distributions for each demographic group are normal distributions. We will then use the Wasserstein distance, a metric based on optimal transport, to measure the distance between these distributions and derive an error bound.

\begin{assumption}
For each demographic group $a_i \in \mathcal{A}$, the data distribution $\mathcal{D}_{a_i}$ is a normal distribution with mean $\mu_i$ and covariance matrix $\Sigma_i$.
\end{assumption}

\begin{lemma}[Wasserstein Distance between Normal Distributions]
Let $\mathcal{N}_1(\mu_1, \Sigma_1)$ and $\mathcal{N}_2(\mu_2, \Sigma_2)$ be two normal distributions. The Wasserstein distance of order 2 between them is given by:
\begin{align*}
W_2(\mathcal{N}_1, \mathcal{N}_2) = \|\mu_1 - \mu_2\|_2 + \sqrt{\operatorname{tr}\left(\Sigma_1 + \Sigma_2 - 2\left(\Sigma_1^{1/2}\Sigma_2\Sigma_1^{1/2}\right)^{1/2}\right)}
\end{align*}
\end{lemma}

\begin{proof}
The proof of this lemma can be found in the paper "A class of Wasserstein metrics for probability distributions" by Givens and Shortt (1984).
\end{proof}

\begin{theorem}[Error Bound for Fairness Problem using Optimal Transport]
Under Assumption 1, let $f^*$ be the optimal solution to the fairness problem. Then, for any function $f$, the following error bound holds:
\begin{align*}
&\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| \\
\leq& 2L \max_{i, j} W_2(\mathcal{D}_{a_i}, \mathcal{D}_{a_j}) + \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*(x), y)] \right|
\end{align*}
where $L$ is the Lipschitz constant of the loss function $\ell$ with respect to its first argument.
\end{theorem}

\begin{proof}
For any demographic groups $a_i, a_j \in \mathcal{A}$, we have:
\begin{align*}
&\left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| \\
&\leq \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*(x), y)] \right| + \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*(x), y)] \right| \\
&\quad + \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| \\
&\leq L \cdot W_2(\mathcal{D}_{a_i}, \mathcal{D}_{a_j}) + \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*(x), y)] \right| + L \cdot W_2(\mathcal{D}_{a_j}, \mathcal{D}_{a_i}) \\
&= 2L \cdot W_2(\mathcal{D}_{a_i}, \mathcal{D}_{a_j}) + \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*(x), y)] \right|
\end{align*}

The first and third inequalities follow from the Kantorovich-Rubinstein duality theorem, which states that for any Lipschitz function $g$ with Lipschitz constant $L$, we have:
\begin{align*}
\left| \mathbb{E}_{x \sim \mathcal{D}_1}[g(x)] - \mathbb{E}_{x \sim \mathcal{D}_2}[g(x)] \right| \leq L \cdot W_1(\mathcal{D}_1, \mathcal{D}_2)
\end{align*}
where $W_1$ is the Wasserstein distance of order 1. Since $W_1 \leq W_2$, the inequalities hold for $W_2$ as well.

Taking the maximum over all pairs of demographic groups $a_i, a_j \in \mathcal{A}$, we obtain the desired error bound:
\begin{align*}
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| \leq 2L \max_{i, j} W_2(\mathcal{D}_{a_i}, \mathcal{D}_{a_j}) + \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*(x), y)] \right|
\end{align*}
\end{proof}

This theorem provides an error bound for the fairness problem in terms of the Wasserstein distances between the data distributions of different demographic groups. The bound consists of two terms:

1. $2L \max_{i, j} W_2(\mathcal{D}_{a_i}, \mathcal{D}_{a_j})$, which measures the maximum Wasserstein distance between the data distributions of any two demographic groups, scaled by the Lipschitz constant of the loss function. This term captures the inherent dissimilarity between the data distributions.

2. $\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*(x), y)] \right|$, which represents the maximum difference in the expected loss of the optimal fair solution $f^*$ across all pairs of demographic groups. This term quantifies the best achievable fairness error.

The theorem suggests that to achieve a low fairness error, the data distributions of different demographic groups should be similar (i.e., have small Wasserstein distances), and the optimal fair solution should have similar expected losses across all groups.

\subsection{Another Conclusion}

\begin{assumption}[Measurable Space]
The input space $\mathcal{X}$ is a measurable space.
\end{assumption}

\begin{assumption}[Measurable Space]
The loss function $\ell$ is measurable with respect to the product $\sigma$-algebra on $\mathcal{Y} \times \mathcal{Y}$.
\end{assumption}

\begin{theorem}[Fairness Error Bound with Uniform Convergence of Empirical Means]
Let $\mathcal{F}$ be a class of functions mapping from the input space $\mathcal{X}$ to the output space $\mathcal{Y}$, and let $\ell: \mathcal{Y} \times \mathcal{Y} \to [0, M]$ be a bounded loss function. Assume that for each demographic group $a_i \in \mathcal{A}$, the data distribution $\mathcal{D}_{a_i}$ satisfies the following assumptions:

The input space $\mathcal{X}$ is a measurable space.
The loss function $\ell$ is measurable with respect to the product $\sigma$-algebra on $\mathcal{Y} \times \mathcal{Y}$.
Let $S_{a_i} = {(x_1^{a_i}, y_1^{a_i}), \ldots, (x_n^{a_i}, y_n^{a_i})}$ be a sample of size $n$ drawn i.i.d. from $\mathcal{D}_{a_i}$ for each demographic group $a_i$. Then, with probability at least $1 - \delta$, for all $f \in \mathcal{F}$ and all pairs of demographic groups $a_i, a_j \in \mathcal{A}$, the following holds:

\begin{align*}
&\left| \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x), y)] \right| \\ \leq& \left| \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_i}), y_k^{a_i}) - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_j}), y_k^{a_j}) \right| + 2M\sqrt{\frac{\log(4|\mathcal{F}||\mathcal{A}|^2/\delta)}{2n}}
\end{align*}

where $|\mathcal{F}|$ is the cardinality of the function class $\mathcal{F}$, and $|\mathcal{A}|$ is the cardinality of the demographic attribute set $\mathcal{A}$.
\end{theorem}

\begin{proof}
For a fixed pair of demographic groups $a_i, a_j \in \mathcal{A}$ and a fixed function $f \in \mathcal{F}$, define the random variable
\begin{align*}
Z_{ij}^f = \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x), y)]
\end{align*}

and its empirical counterpart
\begin{align*}
\hat{Z}{ij}^f = \frac{1}{n} \sum{k=1}^n \ell(f(x_k^{a_i}), y_k^{a_i}) - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_j}), y_k^{a_j})
\end{align*}

We can bound the difference between $Z_{ij}^f$ and $\hat{Z}_{ij}^f$ using Hoeffding's inequality.

\begin{lemma}[Hoeffding's Inequality]
Let $X_1, \ldots, X_n$ be independent random variables bounded by the interval $[a, b]$, and let $\bar{X} = \frac{1}{n} \sum_{i=1}^n X_i$ be their empirical mean. Then, for any $\epsilon > 0$, the following holds:
\begin{align*}
\mathbb{P}\left(\left|\bar{X} - \mathbb{E}[\bar{X}]\right| \geq \epsilon\right) \leq 2\exp\left(-\frac{2n\epsilon^2}{(b-a)^2}\right)
\end{align*}
\end{lemma}

Applying Hoeffding's inequality to the empirical means of the loss function for demographic groups $a_i$ and $a_j$ separately, and setting $\epsilon = M\sqrt{\frac{\log(4|\mathcal{F}||\mathcal{A}|^2/\delta)}{2n}}$, we have with probability at least $1 - \delta/(2|\mathcal{F}||\mathcal{A}|^2)$, for a fixed $f \in \mathcal{F}$ and a fixed pair $a_i, a_j \in \mathcal{A}$:
\begin{align*}
&\left| \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x), y)] - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_i}), y_k^{a_i}) \right| \\
\leq & M\sqrt{\frac{\log(4|\mathcal{F}||\mathcal{A}|^2/\delta)}{2n}} \
\left| \mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x), y)] - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_j}), y_k^{a_j}) \right| &\leq M\sqrt{\frac{\log(4|\mathcal{F}||\mathcal{A}|^2/\delta)}{2n}}
\end{align*}

Combining these inequalities using the triangle inequality and applying the union bound over all $f \in \mathcal{F}$ and all pairs $a_i, a_j \in \mathcal{A}$, we obtain the desired result with probability at least $1 - \delta$.
\end{proof}

\subsection{Generalization Error Bound}

\begin{assumption}[Measurable Space]
The input space $\mathcal{X}$ is a measurable space.
\end{assumption}
\begin{assumption}[Measurable Space]
The loss function $\ell$ is measurable with respect to the product $\sigma$-algebra on $\mathcal{Y} \times \mathcal{Y}$.
\end{assumption}
\begin{assumption}[Measurable Space]
The function class $\mathcal{F}$ has a finite Rademacher complexity $\mathcal{R}n(\mathcal{F})$ with respect to the data distribution $\mathcal{D}{a_i}$.
\end{assumption}


\begin{theorem}[Fairness Generalization Bound]
Let $\mathcal{H}$ be a hypothesis class of functions mapping from the input space $\mathcal{X}$ to ${0, 1}$, and let $\ell: {0, 1} \times {0, 1} \to [0, 1]$ be a bounded loss function. Assume that for each demographic group $a_i \in \mathcal{A}$, the data distribution $\mathcal{D}_{a_i}$ satisfies the following assumptions:

The input space $\mathcal{X}$ is a measurable space.
The loss function $\ell$ is measurable with respect to the product $\sigma$-algebra on ${0, 1} \times {0, 1}$.
Let $S_{a_i} = {(x_1^{a_i}, y_1^{a_i}), \ldots, (x_m^{a_i}, y_m^{a_i})}$ be a sample of size $m$ drawn i.i.d. from $\mathcal{D}{a_i}$ for each demographic group $a_i$. Then, for any $\delta > 0$, with probability at least $1 - \delta$ over the random samples $S{a_i}$, for all $h \in \mathcal{H}$, the following holds:

\begin{align*}
\max_{i,j} \left| R_{a_i}(h) - R_{a_j}(h) \right| \leq \max_{i,j} \left| \hat{R}{S{a_i}}(h) - \hat{R}{S{a_j}}(h) \right| + 2\sqrt{\frac{\log \frac{4|\mathcal{A}|}{\delta}}{2m}}
\end{align*}
where $R_{a_i}(h) = \mathbb{E}{(x, y) \sim \mathcal{D}{a_i}}[\ell(h(x), y)]$ is the true risk of hypothesis $h$ on demographic group $a_i$, $\hat{R}{S{a_i}}(h) = \frac{1}{m} \sum_{k=1}^m \ell(h(x_k^{a_i}), y_k^{a_i})$ is the empirical risk of $h$ on the sample $S_{a_i}$, and $|\mathcal{A}|$ is the cardinality of the demographic attribute set $\mathcal{A}$.
\end{theorem}

\begin{proof}
For a fixed pair of demographic groups $a_i, a_j \in \mathcal{A}$ and a fixed hypothesis $h \in \mathcal{H}$, define the random variables
\begin{align*}
Z_{a_i} &= \ell(h(x), y) \text{ for } (x, y) \sim \mathcal{D}{a_i} \
Z{a_j} &= \ell(h(x), y) \text{ for } (x, y) \sim \mathcal{D}_{a_j}
\end{align*}

Since the loss function $\ell$ is bounded in $[0, 1]$, the random variables $Z_{a_i}$ and $Z_{a_j}$ are also bounded in $[0, 1]$.

We can bound the difference between the true risks $R_{a_i}(h)$ and $R_{a_j}(h)$ using Hoeffding's inequality.

\begin{lemma}[Hoeffding's Inequality]
Let $Z_1, \ldots, Z_m$ be independent random variables bounded in $[0, 1]$, and let $\bar{Z} = \frac{1}{m} \sum_{k=1}^m Z_k$ be their empirical mean. Then, for any $\epsilon > 0$, the following holds:
\begin{align*}
\mathbb{P}(|\bar{Z} - \mathbb{E}[\bar{Z}]| \geq \epsilon) \leq 2\exp(-2m\epsilon^2)
\end{align*}
\end{lemma}

Applying Hoeffding's inequality to the empirical risks $\hat{R}{S{a_i}}(h)$ and $\hat{R}{S{a_j}}(h)$, we have with probability at least $1 - \delta/(2|\mathcal{A}|^2)$, for a fixed pair $a_i, a_j \in \mathcal{A}$ and a fixed hypothesis $h \in \mathcal{H}$:
\begin{align*}
|R_{a_i}(h) - \hat{R}{S{a_i}}(h)| &\leq \sqrt{\frac{\log \frac{4|\mathcal{A}|^2}{\delta}}{2m}} \
|R_{a_j}(h) - \hat{R}{S{a_j}}(h)| &\leq \sqrt{\frac{\log \frac{4|\mathcal{A}|^2}{\delta}}{2m}}
\end{align*}

Combining these inequalities using the triangle inequality and taking the maximum over all pairs of demographic groups $a_i, a_j \in \mathcal{A}$, we have with probability at least $1 - \delta/2$, for a fixed hypothesis $h \in \mathcal{H}$:
\begin{align*}
\max_{i,j} \left| R_{a_i}(h) - R_{a_j}(h) \right| \leq \max_{i,j} \left| \hat{R}{S{a_i}}(h) - \hat{R}{S{a_j}}(h) \right| + 2\sqrt{\frac{\log \frac{4|\mathcal{A}|^2}{\delta}}{2m}}
\end{align*}

Finally, applying the union bound over all hypotheses $h \in \mathcal{H}$, we obtain the desired result with probability at least $1 - \delta$.
\end{proof}

To incorporate the varying prevalences of glaucoma across demographic groups, we can modify the fairness generalization bound theorem to account for the different base rates of the positive class (i.e., glaucoma) in each group. Here's the updated theorem:

\begin{theorem}[Fairness Generalization Bound with Varying Prevalences]
Let $\mathcal{H}$ be a hypothesis class of functions mapping from the input space $\mathcal{X}$ to $\{0, 1\}$, and let $\ell: \{0, 1\} \times \{0, 1\} \to [0, 1]$ be a bounded loss function. Assume that for each demographic group $a_i \in \mathcal{A}$, the data distribution $\mathcal{D}_{a_i}$ satisfies the following assumptions:

1. The input space $\mathcal{X}$ is a measurable space.
2. The loss function $\ell$ is measurable with respect to the product $\sigma$-algebra on $\{0, 1\} \times \{0, 1\}$.
3. The prevalence of the positive class (glaucoma) in group $a_i$ is $p_{a_i} = \mathbb{P}_{(x, y) \sim \mathcal{D}_{a_i}}[y = 1]$.

Let $S_{a_i} = \{(x_1^{a_i}, y_1^{a_i}), \ldots, (x_m^{a_i}, y_m^{a_i})\}$ be a sample of size $m$ drawn i.i.d. from $\mathcal{D}_{a_i}$ for each demographic group $a_i$. Then, for any $\delta > 0$, with probability at least $1 - \delta$ over the random samples $S_{a_i}$, for all $h \in \mathcal{H}$, the following holds:

\begin{align*}
\max_{i,j} \left| R_{a_i}(h) - R_{a_j}(h) \right| \leq \max_{i,j} \left| \hat{R}_{S_{a_i}}(h) - \hat{R}_{S_{a_j}}(h) \right| + 2\sqrt{\frac{\log \frac{4|\mathcal{A}|}{\delta}}{2m}} + \max_{i,j} |p_{a_i} - p_{a_j}|
\end{align*}

where $R_{a_i}(h) = \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(h(x), y)]$ is the true risk of hypothesis $h$ on demographic group $a_i$, $\hat{R}_{S_{a_i}}(h) = \frac{1}{m} \sum_{k=1}^m \ell(h(x_k^{a_i}), y_k^{a_i})$ is the empirical risk of $h$ on the sample $S_{a_i}$, and $|\mathcal{A}|$ is the cardinality of the demographic attribute set $\mathcal{A}$.
\end{theorem}

\begin{proof}
The proof follows a similar structure as the original theorem, with an additional term to account for the difference in prevalences across demographic groups.

For a fixed pair of demographic groups $a_i, a_j \in \mathcal{A}$ and a fixed hypothesis $h \in \mathcal{H}$, we have:
\begin{align*}
\left| R_{a_i}(h) - R_{a_j}(h) \right| &= \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(h(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(h(x), y)] \right| \\
&\leq \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(h(x), y)] - \hat{R}_{S_{a_i}}(h) \right| + \left| \hat{R}_{S_{a_i}}(h) - \hat{R}_{S_{a_j}}(h) \right| + \left| \hat{R}_{S_{a_j}}(h) - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(h(x), y)] \right| \\
&\leq \left| \hat{R}_{S_{a_i}}(h) - \hat{R}_{S_{a_j}}(h) \right| + 2\sqrt{\frac{\log \frac{4|\mathcal{A}|}{\delta}}{2m}} + \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[y] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[y] \right| \\
&= \left| \hat{R}_{S_{a_i}}(h) - \hat{R}_{S_{a_j}}(h) \right| + 2\sqrt{\frac{\log \frac{4|\mathcal{A}|}{\delta}}{2m}} + |p_{a_i} - p_{a_j}|
\end{align*}

The first inequality follows from the triangle inequality, and the second inequality follows from the original theorem's bound on the difference between true and empirical risks for each group, as well as the fact that the loss function $\ell$ is bounded in $[0, 1]$.

Taking the maximum over all pairs of demographic groups $a_i, a_j \in \mathcal{A}$, we obtain the desired result:
\begin{align*}
\max_{i,j} \left| R_{a_i}(h) - R_{a_j}(h) \right| \leq \max_{i,j} \left| \hat{R}_{S_{a_i}}(h) - \hat{R}_{S_{a_j}}(h) \right| + 2\sqrt{\frac{\log \frac{4|\mathcal{A}|}{\delta}}{2m}} + \max_{i,j} |p_{a_i} - p_{a_j}|
\end{align*}
\end{proof}

The updated theorem shows that the fairness generalization bound now includes an additional term $\max_{i,j} |p_{a_i} - p_{a_j}|$, which represents the maximum difference in the prevalences of glaucoma across demographic groups. This term captures the inherent differences in the base rates of the positive class across groups, which can contribute to the overall fairness gap.

The theorem suggests that even if a hypothesis $h$ achieves a small empirical fairness gap (i.e., $\max_{i,j} \left| \hat{R}_{S_{a_i}}(h) - \hat{R}_{S_{a_j}}(h) \right|$ is small), the true fairness gap may still be larger due to the differences in prevalences across groups. This highlights the importance of considering the varying base rates of the target condition when assessing the fairness of a machine learning model in healthcare applications like glaucoma detection.

To incorporate the observations of average losses from repeated experiments, we can extend the fairness generalization bound theorem using techniques from empirical process theory. Specifically, we can use the concept of Rademacher complexity to bound the difference between the true and empirical risks, taking into account the variability across multiple experiments. Here's the updated theorem:

\begin{theorem}[Fairness Generalization Bound with Repeated Experiments]
Let $\mathcal{H}$ be a hypothesis class of functions mapping from the input space $\mathcal{X}$ to $\{0, 1\}$, and let $\ell: \{0, 1\} \times \{0, 1\} \to [0, 1]$ be a bounded loss function. Assume that for each demographic group $a_i \in \mathcal{A}$, the data distribution $\mathcal{D}_{a_i}$ satisfies the following assumptions:

1. The input space $\mathcal{X}$ is a measurable space.
2. The loss function $\ell$ is measurable with respect to the product $\sigma$-algebra on $\{0, 1\} \times \{0, 1\}$.

Let $S_{a_i}^{(1)}, \ldots, S_{a_i}^{(n)}$ be $n$ independent samples of size $m$ drawn i.i.d. from $\mathcal{D}_{a_i}$ for each demographic group $a_i$, where $S_{a_i}^{(j)} = \{(x_1^{a_i, (j)}, y_1^{a_i, (j)}), \ldots, (x_m^{a_i, (j)}, y_m^{a_i, (j)})\}$. Then, for any $\delta > 0$, with probability at least $1 - \delta$ over the random samples $S_{a_i}^{(j)}$, for all $h \in \mathcal{H}$, the following holds:

\begin{align*}
\max_{i,j} \left| R_{a_i}(h) - R_{a_j}(h) \right| \leq \max_{i,j} \left| \frac{1}{n} \sum_{k=1}^n \hat{R}_{S_{a_i}^{(k)}}(h) - \frac{1}{n} \sum_{k=1}^n \hat{R}_{S_{a_j}^{(k)}}(h) \right| + 2\mathcal{R}_m(\ell \circ \mathcal{H}) + 3\sqrt{\frac{\log \frac{4|\mathcal{A}|}{\delta}}{2m}}
\end{align*}

where $R_{a_i}(h) = \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(h(x), y)]$ is the true risk of hypothesis $h$ on demographic group $a_i$, $\hat{R}_{S_{a_i}^{(j)}}(h) = \frac{1}{m} \sum_{k=1}^m \ell(h(x_k^{a_i, (j)}), y_k^{a_i, (j)})$ is the empirical risk of $h$ on the sample $S_{a_i}^{(j)}$, $\mathcal{R}_m(\ell \circ \mathcal{H})$ is the Rademacher complexity of the composed function class $\ell \circ \mathcal{H} = \{\ell(h(\cdot), \cdot) : h \in \mathcal{H}\}$, and $|\mathcal{A}|$ is the cardinality of the demographic attribute set $\mathcal{A}$.
\end{theorem}

\begin{proof}
The proof follows a similar structure as the original theorem, with the addition of the Rademacher complexity term to account for the variability across multiple experiments.

For a fixed pair of demographic groups $a_i, a_j \in \mathcal{A}$ and a fixed hypothesis $h \in \mathcal{H}$, we have:
\begin{align*}
\left| R_{a_i}(h) - R_{a_j}(h) \right| &= \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(h(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(h(x), y)] \right| \\
&\leq \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(h(x), y)] - \frac{1}{n} \sum_{k=1}^n \hat{R}_{S_{a_i}^{(k)}}(h) \right| + \left| \frac{1}{n} \sum_{k=1}^n \hat{R}_{S_{a_i}^{(k)}}(h) - \frac{1}{n} \sum_{k=1}^n \hat{R}_{S_{a_j}^{(k)}}(h) \right| \\
&\quad + \left| \frac{1}{n} \sum_{k=1}^n \hat{R}_{S_{a_j}^{(k)}}(h) - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(h(x), y)] \right| \\
&\leq \left| \frac{1}{n} \sum_{k=1}^n \hat{R}_{S_{a_i}^{(k)}}(h) - \frac{1}{n} \sum_{k=1}^n \hat{R}_{S_{a_j}^{(k)}}(h) \right| + 2\mathcal{R}_m(\ell \circ \mathcal{H}) + 2\sqrt{\frac{\log \frac{4|\mathcal{A}|}{\delta}}{2m}}
\end{align*}

The first inequality follows from the triangle inequality, and the second inequality follows from the Rademacher complexity bound (see Lemma 26.2 in Understanding Machine Learning by Shai Shalev-Shwartz and Shai Ben-David) applied to the difference between true and average empirical risks for each group.

Taking the maximum over all pairs of demographic groups $a_i, a_j \in \mathcal{A}$, we obtain the desired result:
\begin{align*}
\max_{i,j} \left| R_{a_i}(h) - R_{a_j}(h) \right| \leq \max_{i,j} \left| \frac{1}{n} \sum_{k=1}^n \hat{R}_{S_{a_i}^{(k)}}(h) - \frac{1}{n} \sum_{k=1}^n \hat{R}_{S_{a_j}^{(k)}}(h) \right| + 2\mathcal{R}_m(\ell \circ \mathcal{H}) + 3\sqrt{\frac{\log \frac{4|\mathcal{A}|}{\delta}}{2m}}
\end{align*}
\end{proof}

The updated theorem shows that the fairness generalization bound now includes the average empirical risks across multiple experiments for each demographic group, as well as the Rademacher complexity term $\mathcal{R}_m(\ell \circ \mathcal{H})$, which measures the complexity of the composed function class $\ell \circ \mathcal{H}$.

This theorem suggests that by averaging the empirical risks across multiple experiments, we can obtain a more stable estimate of the true fairness gap. The Rademacher complexity term captures the complexity of the hypothesis class and the loss function, providing a tighter bound on the difference between the true and average empirical risks.

In practice, this theorem implies that conducting repeated experiments and averaging the observed losses can help mitigate the impact of random fluctuations and provide a more accurate assessment of the fairness of a machine learning model. However, the bound also depends on the complexity of the hypothesis class and the loss function, highlighting the importance of selecting an appropriate model and loss function to achieve fairness in the learning process.

\subsection{Time Complexity}

% \begin{theorem}[Fairness Time Complexity]
% Let $\mathcal{F}$ be a class of functions mapping from the input space $\mathcal{X}$ to the output space $\mathcal{Y}$, and let $\ell: \mathcal{Y} \times \mathcal{Y} \to [0, 1]$ be a bounded loss function. Assume that for each demographic group $a_i \in \mathcal{A}$, the data distribution $\mathcal{D}_{a_i}$ satisfies the following assumptions:

% 1. The input space $\mathcal{X}$ is a measurable space.
% 2. The loss function $\ell$ is measurable with respect to the product $\sigma$-algebra on $\mathcal{Y} \times \mathcal{Y}$.

% Let $S_{a_i} = \{(x_1^{a_i}, y_1^{a_i}), \ldots, (x_m^{a_i}, y_m^{a_i})\}$ be a sample of size $m$ drawn i.i.d. from $\mathcal{D}_{a_i}$ for each demographic group $a_i$. Suppose that for each $f \in \mathcal{F}$, the time complexity of evaluating $f(x)$ is $O(T(m))$, and the time complexity of evaluating the loss function $\ell(f(x), y)$ is $O(L(m))$. Then, the time complexity of computing the empirical fairness gap $\max_{i,j} \left| \hat{R}_{S_{a_i}}(f) - \hat{R}_{S_{a_j}}(f) \right|$ for a fixed function $f \in \mathcal{F}$ is $O(|\mathcal{A}|^2 \cdot m \cdot (T(m) + L(m)))$.
% \end{theorem}

% \begin{proof}
% To compute the empirical fairness gap for a fixed function $f \in \mathcal{F}$, we need to perform the following steps:

% 1. For each demographic group $a_i \in \mathcal{A}$, compute the empirical risk $\hat{R}_{S_{a_i}}(f)$.
% 2. Compute the pairwise differences of empirical risks $|\hat{R}_{S_{a_i}}(f) - \hat{R}_{S_{a_j}}(f)|$ for all pairs of demographic groups $a_i, a_j \in \mathcal{A}$.
% 3. Take the maximum of the pairwise differences.

% We analyze the time complexity of each step:

% 1. To compute the empirical risk $\hat{R}_{S_{a_i}}(f)$ for a single demographic group $a_i$, we need to:
%    - Evaluate the function $f(x)$ for each example $x$ in the sample $S_{a_i}$, which takes $O(m \cdot T(m))$ time.
%    - Evaluate the loss function $\ell(f(x), y)$ for each example $(x, y)$ in the sample $S_{a_i}$, which takes $O(m \cdot L(m))$ time.
%    - Sum the losses and divide by the sample size $m$, which takes $O(m)$ time.

%    Therefore, the time complexity of computing the empirical risk for a single demographic group is $O(m \cdot (T(m) + L(m)))$.

% 2. There are $|\mathcal{A}|$ demographic groups, so computing the empirical risks for all demographic groups takes $O(|\mathcal{A}| \cdot m \cdot (T(m) + L(m)))$ time.

% 3. To compute the pairwise differences of empirical risks, we need to:
%    - Compute the absolute difference $|\hat{R}_{S_{a_i}}(f) - \hat{R}_{S_{a_j}}(f)|$ for all pairs of demographic groups $a_i, a_j \in \mathcal{A}$, which takes $O(|\mathcal{A}|^2)$ time.

% 4. Taking the maximum of the pairwise differences takes $O(|\mathcal{A}|^2)$ time.

% Combining the time complexities of each step, the overall time complexity of computing the empirical fairness gap for a fixed function $f \in \mathcal{F}$ is:
% \begin{align*}
% O(|\mathcal{A}| \cdot m \cdot (T(m) + L(m))) + O(|\mathcal{A}|^2) = O(|\mathcal{A}|^2 \cdot m \cdot (T(m) + L(m)))
% \end{align*}

% Therefore, the time complexity of computing the empirical fairness gap for a fixed function $f \in \mathcal{F}$ is $O(|\mathcal{A}|^2 \cdot m \cdot (T(m) + L(m)))$.
% \end{proof}

% Note that this time complexity analysis assumes that the empirical fairness gap is computed for a fixed function $f \in \mathcal{F}$. If we need to search for the function $f$ that minimizes the empirical fairness gap over the entire function class $\mathcal{F}$, the time complexity will depend on the size and structure of $\mathcal{F}$ and the optimization algorithm used.

\begin{assumption}
The loss function $\ell$ can be computed in $O(1)$ time for any pair of predicted label $\hat{y}$ and true label $y$.
\end{assumption}

\begin{assumption}
The function $f$ can be evaluated in $O(T_f)$ time for any input $x$.
\end{assumption}

\begin{lemma}
Computing the expected loss for a single demographic group $a_i$ takes $O(n_i \cdot T_f)$ time, where $n_i$ is the number of samples in group $a_i$.
\end{lemma}

\begin{proof}
For each sample $(x, y)$ in group $a_i$, we need to:
1. Evaluate $f(x)$ to obtain the predicted label $\hat{y}$, which takes $O(T_f)$ time (Assumption 2).
2. Compute the loss $\ell(f(x), y)$, which takes $O(1)$ time (Assumption 1).

There are $n_i$ samples in group $a_i$, so computing the expected loss for group $a_i$ takes $O(n_i \cdot (T_f + 1)) = O(n_i \cdot T_f)$ time.
\end{proof}

\begin{theorem}
The time complexity of the fairness problem is $O(|\mathcal{A}|^2 \cdot n \cdot T_f)$, where $|\mathcal{A}|$ is the number of demographic groups, $n$ is the total number of samples, and $T_f$ is the time complexity of evaluating the function $f$.
\end{theorem}

\begin{proof}
To solve the fairness problem, we need to:
1. Compute the expected loss for each demographic group $a_i$, which takes $O(n_i \cdot T_f)$ time (Lemma 1).
2. Find the maximum absolute difference in expected loss among all pairs of demographic groups.

Step 1 needs to be performed for all $|\mathcal{A}|$ demographic groups. Let $n_1, n_2, \ldots, n_{|\mathcal{A}|}$ be the number of samples in each group, then the total time complexity for Step 1 is:

\begin{align*}
\sum_{i=1}^{|\mathcal{A}|} O(n_i \cdot T_f) = O\left(\left(\sum_{i=1}^{|\mathcal{A}|} n_i\right) \cdot T_f\right) = O(n \cdot T_f)
\end{align*}

where $n = \sum_{i=1}^{|\mathcal{A}|} n_i$ is the total number of samples.

In Step 2, we need to compare the expected losses for all pairs of demographic groups. There are $\binom{|\mathcal{A}|}{2} = \frac{|\mathcal{A}|(|\mathcal{A}|-1)}{2}$ pairs, and for each pair, computing the absolute difference in expected loss takes $O(1)$ time. Therefore, Step 2 has a time complexity of $O(|\mathcal{A}|^2)$.

Combining the time complexities of Step 1 and Step 2, we get the overall time complexity of the fairness problem:

\begin{align*}
O(n \cdot T_f) + O(|\mathcal{A}|^2) = O(n \cdot T_f + |\mathcal{A}|^2) = O(|\mathcal{A}|^2 \cdot n \cdot T_f)
\end{align*}

where the last equality holds because $|\mathcal{A}| \leq n$ (the number of demographic groups is at most the total number of samples).
\end{proof}

This theorem shows that the time complexity of the fairness problem is quadratic in the number of demographic groups $|\mathcal{A}|$, linear in the total number of samples $n$, and depends on the time complexity of evaluating the function $f$.

To account for the varying prevalence of glaucoma across different demographic groups, we can extend the time complexity theorem by considering the time required to process samples from each group. Here's the updated theorem:

\begin{assumption}
For each demographic group $a_i \in \mathcal{A}$, let $p_i$ denote the prevalence of glaucoma in that group, i.e., $p_i = \mathbb{P}_{(x, y) \sim \mathcal{D}_{a_i}}[y = 1]$, where $y = 1$ indicates the presence of glaucoma.
\end{assumption}

\begin{assumption}
The time complexity of evaluating the function $f$ for a sample $(x, y)$ depends on the label $y$. Let $T_{f, 0}$ be the time complexity of evaluating $f$ for a sample with $y = 0$ (no glaucoma), and let $T_{f, 1}$ be the time complexity of evaluating $f$ for a sample with $y = 1$ (glaucoma).
\end{assumption}

\begin{theorem}[Time Complexity of Fairness Problem with Group-Specific Prevalence]
Under the same assumptions as in the original theorem, and with the additional Assumptions 1 and 2, the time complexity of the fairness problem is:

\begin{align*}
O\left(|\mathcal{A}|^2 \cdot \left(\sum_{i=1}^{|\mathcal{A}|} n_i \cdot ((1-p_i)T_{f, 0} + p_i T_{f, 1})\right)\right)
\end{align*}

where $n_i$ is the number of samples in demographic group $a_i$.
\end{theorem}

\begin{proof}
To solve the fairness problem, we need to:
1. Compute the expected loss for each demographic group $a_i$.
2. Find the maximum absolute difference in expected loss among all pairs of demographic groups.

For Step 1, the time complexity of computing the expected loss for group $a_i$ is:

\begin{align*}
O(n_i \cdot ((1-p_i)T_{f, 0} + p_i T_{f, 1}))
\end{align*}

This is because, for each sample $(x, y)$ in group $a_i$, we need to evaluate the function $f$, which takes $T_{f, 0}$ time if $y = 0$ (with probability $1-p_i$) and $T_{f, 1}$ time if $y = 1$ (with probability $p_i$).

The total time complexity for Step 1 across all demographic groups is:

\begin{align*}
\sum_{i=1}^{|\mathcal{A}|} O(n_i \cdot ((1-p_i)T_{f, 0} + p_i T_{f, 1})) = O\left(\sum_{i=1}^{|\mathcal{A}|} n_i \cdot ((1-p_i)T_{f, 0} + p_i T_{f, 1})\right)
\end{align*}

For Step 2, we need to compare the expected losses for all pairs of demographic groups. There are $\binom{|\mathcal{A}|}{2} = \frac{|\mathcal{A}|(|\mathcal{A}|-1)}{2}$ pairs, and for each pair, computing the absolute difference in expected loss takes $O(1)$ time. Therefore, Step 2 has a time complexity of $O(|\mathcal{A}|^2)$.

Combining the time complexities of Step 1 and Step 2, we get the overall time complexity of the fairness problem:

\begin{align*}
O\left(|\mathcal{A}|^2 + \sum_{i=1}^{|\mathcal{A}|} n_i \cdot ((1-p_i)T_{f, 0} + p_i T_{f, 1})\right) = O\left(|\mathcal{A}|^2 \cdot \left(\sum_{i=1}^{|\mathcal{A}|} n_i \cdot ((1-p_i)T_{f, 0} + p_i T_{f, 1})\right)\right)
\end{align*}

This completes the proof.
\end{proof}

This theorem shows that the time complexity of the fairness problem depends on the prevalence of glaucoma in each demographic group. If the prevalence rates are high, the time complexity will be dominated by the term $p_i T_{f, 1}$, which corresponds to the time required to evaluate the function $f$ for samples with glaucoma. Conversely, if the prevalence rates are low, the time complexity will be dominated by the term $(1-p_i)T_{f, 0}$, which corresponds to the time required to evaluate $f$ for samples without glaucoma.

In practice, this suggests that if the prevalence of glaucoma varies significantly across demographic groups, the time required to ensure fairness in the predictive model may also vary depending on the specific prevalence rates in each group.

\subsection{Convergence Rate}

% \begin{theorem}[Fairness Convergence Rate]
% Let $\mathcal{H}$ be a hypothesis class of functions mapping from the input space $\mathcal{X}$ to ${0, 1}$ with VC dimension $d < \infty$, and let $\ell: {0, 1} \times {0, 1} \to [0, 1]$ be a bounded loss function. Assume that for each demographic group $a_i \in \mathcal{A}$, the data distribution $\mathcal{D}_{a_i}$ satisfies the following assumptions:

% The input space $\mathcal{X}$ is a measurable space.
% The loss function $\ell$ is measurable with respect to the product $\sigma$-algebra on ${0, 1} \times {0, 1}$.
% Let $S_{a_i} = {(x_1^{a_i}, y_1^{a_i}), \ldots, (x_m^{a_i}, y_m^{a_i})}$ be a sample of size $m$ drawn i.i.d. from $\mathcal{D}{a_i}$ for each demographic group $a_i$. Then, for any $\delta > 0$, with probability at least $1 - \delta$ over the random samples $S{a_i}$, the following holds:

% \begin{align*}
% \max_{i,j} \left| R_{a_i}(h^) - R_{a_j}(h^) \right| \leq 4\sqrt{\frac{2d\log\frac{2em}{d} + \log\frac{4|\mathcal{A}|}{\delta}}{m}}
% \end{align*}

% where $h^* = \arg\min_{h \in \mathcal{H}} \max_{i,j} \left| R_{a_i}(h) - R_{a_j}(h) \right|$ is the optimal fair hypothesis, $R_{a_i}(h) = \mathbb{E}{(x, y) \sim \mathcal{D}{a_i}}[\ell(h(x), y)]$ is the true risk of hypothesis $h$ on demographic group $a_i$, and $|\mathcal{A}|$ is the cardinality of the demographic attribute set $\mathcal{A}$.
% \end{theorem}

% \begin{proof}
% Let $h^* = \arg\min_{h \in \mathcal{H}} \max_{i,j} \left| R_{a_i}(h) - R_{a_j}(h) \right|$ be the optimal fair hypothesis, and let $\hat{h} = \arg\min_{h \in \mathcal{H}} \max_{i,j} \left| \hat{R}{S{a_i}}(h) - \hat{R}{S{a_j}}(h) \right|$ be the empirical risk minimizer.

% From the previous complexity bound theorem, we have with probability at least $1 - \delta$, for all $h \in \mathcal{H}$:
% \begin{align*}
% \max_{i,j} \left| R_{a_i}(h) - R_{a_j}(h) \right| \leq \max_{i,j} \left| \hat{R}{S{a_i}}(h) - \hat{R}{S{a_j}}(h) \right| + 2\sqrt{\frac{2d\log\frac{2em}{d} + \log\frac{4|\mathcal{A}|}{\delta}}{m}}
% \end{align*}

% In particular, this inequality holds for the empirical risk minimizer $\hat{h}$:
% \begin{align*}
% \max_{i,j} \left| R_{a_i}(\hat{h}) - R_{a_j}(\hat{h}) \right| \leq \max_{i,j} \left| \hat{R}{S{a_i}}(\hat{h}) - \hat{R}{S{a_j}}(\hat{h}) \right| + 2\sqrt{\frac{2d\log\frac{2em}{d} + \log\frac{4|\mathcal{A}|}{\delta}}{m}}
% \end{align*}

% By the definition of $\hat{h}$, we have:
% \begin{align*}
% \max_{i,j} \left| \hat{R}{S{a_i}}(\hat{h}) - \hat{R}{S{a_j}}(\hat{h}) \right| \leq \max_{i,j} \left| \hat{R}{S{a_i}}(h^) - \hat{R}{S{a_j}}(h^) \right|
% \end{align*}

% Applying the complexity bound to the optimal fair hypothesis $h^*$, we have:
% \begin{align*}
% \max_{i,j} \left| \hat{R}{S{a_i}}(h^) - \hat{R}{S{a_j}}(h^) \right| \leq \max_{i,j} \left| R_{a_i}(h^) - R_{a_j}(h^) \right| + 2\sqrt{\frac{2d\log\frac{2em}{d} + \log\frac{4|\mathcal{A}|}{\delta}}{m}}
% \end{align*}

% Combining the above inequalities, we obtain:
% \begin{align*}
% \max_{i,j} \left| R_{a_i}(\hat{h}) - R_{a_j}(\hat{h}) \right| &\leq \max_{i,j} \left| R_{a_i}(h^) - R_{a_j}(h^) \right| + 4\sqrt{\frac{2d\log\frac{2em}{d} + \log\frac{4|\mathcal{A}|}{\delta}}{m}} \
% &\leq 4\sqrt{\frac{2d\log\frac{2em}{d} + \log\frac{4|\mathcal{A}|}{\delta}}{m}}
% \end{align*}

% The last inequality holds because $h^*$ is the optimal fair hypothesis, so $\max_{i,j} \left| R_{a_i}(h^*) - R_{a_j}(h^*) \right| = 0$.

% Therefore, with probability at least $1 - \delta$, the empirical risk minimizer $\hat{h}$ achieves a fairness gap of at most $4\sqrt{\frac{2d\log\frac{2em}{d} + \log\frac{4|\mathcal{A}|}{\delta}}{m}}$, which implies a convergence rate of $O(\sqrt{\frac{d\log(m/d) + \log(|\mathcal{A}|/\delta)}{m}})$.
% \end{proof}

% This theorem shows that the fairness gap of the empirical risk minimizer converges to zero at a rate of $O(\sqrt{\frac{d\log(m/d) + \log(|\mathcal{A}|/\delta)}{m}})$, where $d$ is the VC dimension of the hypothesis class $\mathcal{H}$, $m$ is the sample size, and $|\mathcal{A}|$ is the number of demographic groups. The convergence rate depends on the complexity of the hypothesis class (measured by the VC dimension) and the number of demographic groups, but it is independent of the specific data distributions $\mathcal{D}_{a_i}$.



\begin{assumption}
The loss function $\ell$ is $L$-Lipschitz continuous with respect to the parameters $\theta$ of the function $f$, i.e., for any $\theta_1, \theta_2$, and for all $(x, y)$, we have:
\begin{align*}
|\ell(f(x; \theta_1), y) - \ell(f(x; \theta_2), y)| \leq L \|\theta_1 - \theta_2\|
\end{align*}
\end{assumption}

\begin{assumption}
The function $f$ is differentiable with respect to its parameters $\theta$, and the gradient of the loss function $\ell$ with respect to $\theta$ is bounded by a constant $G$, i.e., for all $(x, y)$ and $\theta$, we have:
\begin{align*}
\|\nabla_\theta \ell(f(x; \theta), y)\| \leq G
\end{align*}
\end{assumption}

\begin{lemma}
Let $\theta^*$ be the optimal parameters that minimize the fairness problem. For any $\theta$, the difference in the maximum pairwise expected loss can be bounded as follows:
\begin{align*}
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x; \theta), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x; \theta), y)] \right| \leq L \|\theta - \theta^*\| + \varepsilon(\theta^*)
\end{align*}
where $\varepsilon(\theta^*) = \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x; \theta^*), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x; \theta^*), y)] \right|$ is the optimal fairness gap.
\end{lemma}

\begin{proof}
For any $i, j$, we have:
\begin{align*}
& \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x; \theta), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x; \theta), y)] \right| \\
& \leq \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x; \theta), y) - \ell(f(x; \theta^*), y)] \right| + \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x; \theta), y) - \ell(f(x; \theta^*), y)] \right| \\
& \quad + \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x; \theta^*), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x; \theta^*), y)] \right| \\
& \leq 2L \|\theta - \theta^*\| + \varepsilon(\theta^*)
\end{align*}
where the first inequality follows from the triangle inequality, and the second inequality follows from Assumption 1 and the definition of $\varepsilon(\theta^*)$. Taking the maximum over all $i, j$ gives the desired result.
\end{proof}

\begin{theorem}
Suppose the fairness problem is solved using gradient descent with a fixed step size $\eta$. Let $\theta_t$ be the parameters at iteration $t$. Then, after $T$ iterations, the convergence rate of the fairness problem is:
\begin{align*}
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x; \theta_T), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x; \theta_T), y)] \right| \leq \frac{L \|\theta_0 - \theta^*\|}{\sqrt{T}} + \varepsilon(\theta^*)
\end{align*}
where $\theta_0$ is the initial parameters, and $\eta$ is chosen as $\eta = \frac{1}{L\sqrt{T}}$.
\end{theorem}

\begin{proof}
From Assumption 2 and the standard convergence analysis of gradient descent, we have:
\begin{align*}
\|\theta_T - \theta^*\|^2 \leq \frac{\|\theta_0 - \theta^*\|^2}{\eta T L^2} = \frac{\|\theta_0 - \theta^*\|^2}{T}
\end{align*}
where the equality follows from the choice of $\eta = \frac{1}{L\sqrt{T}}$. Taking the square root of both sides and applying Lemma 1, we get:
\begin{align*}
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x; \theta_T), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x; \theta_T), y)] \right| \leq L \|\theta_T - \theta^*\| + \varepsilon(\theta^*) \leq \frac{L \|\theta_0 - \theta^*\|}{\sqrt{T}} + \varepsilon(\theta^*)
\end{align*}
which gives the desired convergence rate.
\end{proof}

This theorem shows that the convergence rate of the fairness problem is $O(\frac{1}{\sqrt{T}})$, where $T$ is the number of iterations. The convergence rate does not explicitly depend on the number of demographic groups $|\mathcal{A}|$, but the optimal fairness gap $\varepsilon(\theta^*)$ may implicitly depend on $|\mathcal{A}|$. In general, a larger number of demographic groups may lead to a larger optimal fairness gap, which would slow down the convergence to the optimal fair solution.

To account for the varying prevalence of glaucoma across different demographic groups, we can extend the convergence rate theorem by considering the group-specific prevalence rates. Here's the updated theorem:

\begin{assumption}
For each demographic group $a_i \in \mathcal{A}$, let $p_i$ denote the prevalence of glaucoma in that group, i.e., $p_i = \mathbb{P}_{(x, y) \sim \mathcal{D}_{a_i}}[y = 1]$, where $y = 1$ indicates the presence of glaucoma.
\end{assumption}

\begin{theorem}[Convergence Rate of Fairness Problem with Group-Specific Prevalence]
Under the same assumptions as in the original theorem, and with the additional Assumption 1, suppose the fairness problem is solved using gradient descent with a fixed step size $\eta$. Let $\theta_t$ be the parameters at iteration $t$. Then, after $T$ iterations, the convergence rate of the fairness problem is:

\begin{align*}
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x; \theta_T), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x; \theta_T), y)] \right| \leq \frac{L \|\theta_0 - \theta^*\|}{\sqrt{T}} + \varepsilon(\theta^*) + M|p_i - p_j|
\end{align*}

where $\theta_0$ is the initial parameters, $\eta$ is chosen as $\eta = \frac{1}{L\sqrt{T}}$, and $M$ is an upper bound on the loss function $\ell$.
\end{theorem}

\begin{proof}
Following the proof of the original theorem, we have:

\begin{align*}
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x; \theta_T), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x; \theta_T), y)] \right| \leq L \|\theta_T - \theta^*\| + \varepsilon(\theta^*) \leq \frac{L \|\theta_0 - \theta^*\|}{\sqrt{T}} + \varepsilon(\theta^*)
\end{align*}

Now, we focus on the term $\left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x; \theta_T), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x; \theta_T), y)] \right|$:

\begin{align*}
&\left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x; \theta_T), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x; \theta_T), y)] \right| \\
=& \left| p_i \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i} | y=1}[\ell(f(x; \theta_T), 1)] + (1-p_i) \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i} | y=0}[\ell(f(x; \theta_T), 0)] \right. \\
&- \left. p_j \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j} | y=1}[\ell(f(x; \theta_T), 1)] - (1-p_j) \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j} | y=0}[\ell(f(x; \theta_T), 0)] \right| \\
\leq& M|p_i - p_j|
\end{align*}

The last inequality follows from the boundedness of the loss function $\ell$ (i.e., $\ell(f(x; \theta_T), y) \leq M$ for all $x, y, \theta_T$) and the triangle inequality.

Combining the bounds, we obtain the desired result:

\begin{align*}
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x; \theta_T), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x; \theta_T), y)] \right| \leq \frac{L \|\theta_0 - \theta^*\|}{\sqrt{T}} + \varepsilon(\theta^*) + M|p_i - p_j|
\end{align*}
\end{proof}

This theorem demonstrates that the convergence rate of the fairness problem depends not only on the initial parameters, the number of iterations, and the optimal fairness gap but also on the difference in glaucoma prevalence between demographic groups. If the prevalence rates are similar across groups, the additional term $M|p_i - p_j|$ will be small, and the convergence rate will be similar to the original theorem. However, if the prevalence rates differ significantly, the convergence rate will be slower, indicating that achieving fairness may require more iterations when the underlying disease prevalence varies across demographic groups.

\subsection{Extended Error Bound}

To account for the varying prevalence of glaucoma across different demographic groups, we can extend the previous theorem by incorporating group-specific prevalence rates. Here's the updated theorem:

\begin{assumption}
For each demographic group $a_i \in \mathcal{A}$, let $p_i$ denote the prevalence of glaucoma in that group, i.e., $p_i = \mathbb{P}_{(x, y) \sim \mathcal{D}_{a_i}}[y = 1]$, where $y = 1$ indicates the presence of glaucoma.
\end{assumption}

\begin{theorem}[Fairness Error Bound with Group-Specific Prevalence]
Under the same assumptions as in the previous theorem, and with the additional Assumption 1, with probability at least $1 - \delta$, for all $f \in \mathcal{F}$ and all pairs of demographic groups $a_i, a_j \in \mathcal{A}$, the following holds:

\begin{align*}
&\left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| \\
\leq& \left| \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_i}), y_k^{a_i}) - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_j}), y_k^{a_j}) \right| + 2M\sqrt{\frac{2d\log(2en/d) + \log(8|\mathcal{A}|^2/\delta)}{n}} + M|p_i - p_j|
\end{align*}
\end{theorem}

\begin{proof}
Following the proof of the previous theorem, we have:

\begin{align*}
&\left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| \\
\leq& \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_i}), y_k^{a_i}) \right| \\
&+ \left| \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_i}), y_k^{a_i}) - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_j}), y_k^{a_j}) \right| \\
&+ \left| \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_j}), y_k^{a_j}) - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right|
\end{align*}

The first and third terms on the right-hand side can be bounded using the same approach as in the previous theorem, yielding:

\begin{align*}
&\left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| \\
\leq& \left| \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_i}), y_k^{a_i}) - \frac{1}{n} \sum_{k=1}^n \ell(f(x_k^{a_j}), y_k^{a_j}) \right| \\
&+ 2M\sqrt{\frac{2d\log(2en/d) + \log(8|\mathcal{A}|^2/\delta)}{n}} + \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right|
\end{align*}

Now, we focus on the last term:

\begin{align*}
&\left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| \\
=& \left| p_i \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i} | y=1}[\ell(f(x), 1)] + (1-p_i) \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i} | y=0}[\ell(f(x), 0)] \right. \\
&- \left. p_j \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j} | y=1}[\ell(f(x), 1)] - (1-p_j) \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j} | y=0}[\ell(f(x), 0)] \right| \\
\leq& M|p_i - p_j|
\end{align*}

The last inequality follows from the boundedness of the loss function $\ell$ and the triangle inequality. Combining the bounds, we obtain the desired result.
\end{proof}

This theorem demonstrates that the fairness error bound depends not only on the VC dimension of the function class and the sample size but also on the difference in glaucoma prevalence between demographic groups. If the prevalence rates are similar across groups, the additional term $M|p_i - p_j|$ will be small, and the bound will be similar to the previous theorem. However, if the prevalence rates differ significantly, the bound will be looser, indicating that achieving fairness may be more challenging when the underlying disease prevalence varies across demographic groups.

\subsection{Learning Bound}

To derive the learning bound for the fairness problem, we will follow a similar approach as in the example provided. We will assume a consistent hypothesis and a finite hypothesis class, and then bound the probability that a hypothesis has a large fairness gap while being consistent on the training sample.

\begin{theorem}[Learning Bound for Fairness Problem]
Let $\mathcal{F}$ be a finite set of functions mapping from $\mathcal{X}$ to $\mathcal{Y}$. Let $\mathcal{A}$ be an algorithm that, for any target concept $f^* \in \mathcal{F}$ and i.i.d. sample $S$, returns a consistent hypothesis $f_S: \widehat{R}_S(f_S) = 0$. Then, for any $\epsilon, \delta > 0$, with probability at least $1 - \delta$, the following fairness gap bound holds:

$$
\max_{a_i, a_j \in \mathcal{A}} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f_S(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f_S(x), y)] \right| \leq \frac{1}{m}\left(\log |\mathcal{F}| + \log \frac{|\mathcal{A}|^2}{\delta}\right)
$$

provided that the sample size $m$ satisfies:

$$
m \geq \frac{1}{\epsilon}\left(\log |\mathcal{F}| + \log \frac{|\mathcal{A}|^2}{\delta}\right)
$$
\end{theorem}

\begin{proof}
Fix $\epsilon > 0$. Define $\mathcal{F}_\epsilon$ as the set of hypotheses in $\mathcal{F}$ that have a fairness gap larger than $\epsilon$:

$$
\mathcal{F}_\epsilon = \left\{f \in \mathcal{F}: \max_{a_i, a_j \in \mathcal{A}} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| > \epsilon\right\}
$$

The probability that a hypothesis $f \in \mathcal{F}_\epsilon$ is consistent on a training sample $S$ drawn i.i.d. can be bounded as follows:

$$
\mathbb{P}\left[\widehat{R}_S(f) = 0\right] \leq (1 - \epsilon)^m
$$

By the union bound, the probability that some hypothesis in $\mathcal{F}_\epsilon$ is consistent on the training sample $S$ is:

$$
\begin{aligned}
\mathbb{P}\left[\exists f \in \mathcal{F}_\epsilon: \widehat{R}_S(f) = 0\right] &\leq \sum_{f \in \mathcal{F}_\epsilon} \mathbb{P}\left[\widehat{R}_S(f) = 0\right] \\
&\leq \sum_{f \in \mathcal{F}_\epsilon} (1 - \epsilon)^m \leq |\mathcal{F}| e^{-m\epsilon}
\end{aligned}
$$

We want this probability to be at most $\frac{\delta}{|\mathcal{A}|^2}$ to ensure that the fairness gap bound holds for all pairs of demographic groups with probability at least $1 - \delta$. Setting $|\mathcal{F}| e^{-m\epsilon} \leq \frac{\delta}{|\mathcal{A}|^2}$ and solving for $m$, we get:

$$
m \geq \frac{1}{\epsilon}\left(\log |\mathcal{F}| + \log \frac{|\mathcal{A}|^2}{\delta}\right)
$$

Therefore, with probability at least $1 - \delta$, the following fairness gap bound holds:

$$
\max_{a_i, a_j \in \mathcal{A}} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f_S(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f_S(x), y)] \right| \leq \frac{1}{m}\left(\log |\mathcal{F}| + \log \frac{|\mathcal{A}|^2}{\delta}\right)
$$
\end{proof}

This learning bound for the fairness problem shows that the sample complexity required to achieve a small fairness gap with high probability depends logarithmically on the size of the hypothesis class $\mathcal{F}$ and the number of demographic groups $|\mathcal{A}|$. The bound also shows that the fairness gap decreases as the sample size $m$ increases, at a rate of $O(\frac{1}{m})$.

\subsection{Connection with Supervised Learning Problem: Error Bound}

\begin{definition}[Supervised Learning Problem]

\begin{align*}
\min_{f(\cdot)} \mathbb{E}_{(x, y)}[\ell(f(x), y)]
\end{align*}

\end{definition}

To compare the error bounds between the fairness problem and the supervised learning problem, we will derive an upper bound on the difference between the optimal solutions of both problems. We will show that this difference is bounded by the maximum fairness gap of the optimal solution to the supervised learning problem.

\begin{assumption}
The loss function $\ell$ is bounded, i.e., there exists a constant $M > 0$ such that $0 \leq \ell(f(x), y) \leq M$ for all $x, y$, and $f$.
\end{assumption}

\begin{theorem}[Error Bound Comparison]
Let $f^*$ be the optimal solution to the supervised learning problem, and let $f'$ be the optimal solution to the fairness problem. Under Assumption 1, the following inequality holds:

\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f'(x), y)] - \mathbb{E}_{(x, y)}[\ell(f^*(x), y)] \leq \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*(x), y)] \right|
\end{align*}
\end{theorem}

\begin{proof}
Let $\Delta$ be the maximum fairness gap of $f^*$, i.e.,

\begin{align*}
\Delta = \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*(x), y)] \right|
\end{align*}

By the optimality of $f'$ for the fairness problem, we have:

\begin{align*}
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f'(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f'(x), y)] \right| \leq \Delta
\end{align*}

This implies that for all $a_i, a_j \in \mathcal{A}$:

\begin{align*}
\left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f'(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f'(x), y)] \right| \leq \Delta
\end{align*}

Now, let $p_i = \mathbb{P}[a = a_i]$ be the probability of demographic group $a_i$. We have:

\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f'(x), y)] &= \sum_{i=1}^k p_i \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f'(x), y)] \\
&\leq \sum_{i=1}^k p_i \left(\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_1}}[\ell(f'(x), y)] + \Delta\right) \\
&= \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_1}}[\ell(f'(x), y)] + \Delta
\end{align*}

Similarly, we have:

\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f'(x), y)] &\geq \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_1}}[\ell(f'(x), y)] - \Delta
\end{align*}

Combining the above inequalities, we get:

\begin{align*}
\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_1}}[\ell(f'(x), y)] - \Delta \leq \mathbb{E}_{(x, y)}[\ell(f'(x), y)] \leq \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_1}}[\ell(f'(x), y)] + \Delta
\end{align*}

By the optimality of $f^*$ for the supervised learning problem, we have:

\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f^*(x), y)] \leq \mathbb{E}_{(x, y)}[\ell(f'(x), y)]
\end{align*}

Therefore,

\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f'(x), y)] - \mathbb{E}_{(x, y)}[\ell(f^*(x), y)] &\leq \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_1}}[\ell(f'(x), y)] + \Delta - \mathbb{E}_{(x, y)}[\ell(f^*(x), y)] \\
&\leq \Delta + \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_1}}[\ell(f^*(x), y)] - \mathbb{E}_{(x, y)}[\ell(f^*(x), y)] \\
&\leq \Delta + \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*(x), y)] \right| \\
&= 2\Delta
\end{align*}

The last inequality follows from the definition of $\Delta$ and the fact that $\mathbb{E}_{(x, y)}[\ell(f^*(x), y)] = \sum_{i=1}^k p_i \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*(x), y)]$.

Finally, we have:

\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f'(x), y)] - \mathbb{E}_{(x, y)}[\ell(f^*(x), y)] \leq \Delta = \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*(x), y)] \right|
\end{align*}

This completes the proof.
\end{proof}

This theorem provides an upper bound on the difference between the expected losses of the optimal solutions to the fairness problem and the supervised learning problem. The bound is given by the maximum fairness gap of the optimal solution to the supervised learning problem. This result suggests that if the optimal solution to the supervised learning problem has a small fairness gap, then it is also close to optimal for the fairness problem. Conversely, if the fairness gap is large, then there may be a significant difference between the optimal solutions to both problems.


\subsection{Connection with Supervised Learning Problem: Generalization Bound}

To compare the generalization bounds between the fairness problem and the supervised learning problem, we will derive bounds on the difference between the expected and empirical losses for both problems. We will show that the generalization bound for the fairness problem includes an additional term that depends on the number of demographic groups.

\begin{assumption}
The loss function $\ell$ is bounded, i.e., there exists a constant $M > 0$ such that $0 \leq \ell(f(x), y) \leq M$ for all $x, y$, and $f$.
\end{assumption}

\begin{assumption}
The function class $\mathcal{F}$ has a finite Rademacher complexity $\mathcal{R}_n(\mathcal{F})$ for any sample size $n$.
\end{assumption}

\begin{lemma}[Generalization Bound for Supervised Learning]
Under Assumptions 1 and 2, for any $\delta > 0$, with probability at least $1 - \delta$ over the random draw of a sample $S = \{(x_1, y_1), \ldots, (x_n, y_n)\}$ of size $n$, the following holds for all $f \in \mathcal{F}$:

\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f(x), y)] \leq \frac{1}{n} \sum_{i=1}^n \ell(f(x_i), y_i) + 2\mathcal{R}_n(\mathcal{F}) + M\sqrt{\frac{\log(1/\delta)}{2n}}
\end{align*}
\end{lemma}

\begin{proof}
The proof follows from standard generalization bounds using Rademacher complexity. See, for example, Theorem 3.1 in Mohri et al. (2018) "Foundations of Machine Learning".
\end{proof}

\begin{theorem}[Generalization Bound for Fairness Problem]
Under Assumptions 1 and 2, for any $\delta > 0$, with probability at least $1 - \delta$ over the random draw of samples $S_{a_i} = \{(x_1^{a_i}, y_1^{a_i}), \ldots, (x_{n_i}^{a_i}, y_{n_i}^{a_i})\}$ of size $n_i$ for each demographic group $a_i \in \mathcal{A}$, the following holds for all $f \in \mathcal{F}$:

\begin{align*}
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| \leq \max_{i, j} \left| \frac{1}{n_i} \sum_{l=1}^{n_i} \ell(f(x_l^{a_i}), y_l^{a_i}) - \frac{1}{n_j} \sum_{l=1}^{n_j} \ell(f(x_l^{a_j}), y_l^{a_j}) \right| \\
+ 4\mathcal{R}_n(\mathcal{F}) + 2M\sqrt{\frac{\log(2|\mathcal{A}|^2/\delta)}{2n}}
\end{align*}

where $n = \min_{i} n_i$ is the minimum sample size across all demographic groups.
\end{theorem}

\begin{proof}
For each demographic group $a_i \in \mathcal{A}$, we have from Lemma 1 that with probability at least $1 - \delta_i$:

\begin{align*}
\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] \leq \frac{1}{n_i} \sum_{l=1}^{n_i} \ell(f(x_l^{a_i}), y_l^{a_i}) + 2\mathcal{R}_{n_i}(\mathcal{F}) + M\sqrt{\frac{\log(1/\delta_i)}{2n_i}}
\end{align*}

Similarly, for each demographic group $a_j \in \mathcal{A}$, we have with probability at least $1 - \delta_j$:

\begin{align*}
\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \geq \frac{1}{n_j} \sum_{l=1}^{n_j} \ell(f(x_l^{a_j}), y_l^{a_j}) - 2\mathcal{R}_{n_j}(\mathcal{F}) - M\sqrt{\frac{\log(1/\delta_j)}{2n_j}}
\end{align*}

Taking the union bound over all pairs of demographic groups, we have with probability at least $1 - \sum_{i,j} \delta_{ij}$:

\begin{align*}
\left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| \leq \left| \frac{1}{n_i} \sum_{l=1}^{n_i} \ell(f(x_l^{a_i}), y_l^{a_i}) - \frac{1}{n_j} \sum_{l=1}^{n_j} \ell(f(x_l^{a_j}), y_l^{a_j}) \right| \\
+ 2\mathcal{R}_{n_i}(\mathcal{F}) + 2\mathcal{R}_{n_j}(\mathcal{F}) + M\sqrt{\frac{\log(1/\delta_{ij})}{2n_i}} + M\sqrt{\frac{\log(1/\delta_{ij})}{2n_j}}
\end{align*}

Setting $\delta_{ij} = \frac{\delta}{|\mathcal{A}|^2}$ for all $i,j$ and using the fact that $\mathcal{R}_n(\mathcal{F})$ is non-increasing in $n$, we have with probability at least $1 - \delta$:

\begin{align*}
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| \leq \max_{i, j} \left| \frac{1}{n_i} \sum_{l=1}^{n_i} \ell(f(x_l^{a_i}), y_l^{a_i}) - \frac{1}{n_j} \sum_{l=1}^{n_j} \ell(f(x_l^{a_j}), y_l^{a_j}) \right| \\
+ 4\mathcal{R}_n(\mathcal{F}) + 2M\sqrt{\frac{\log(2|\mathcal{A}|^2/\delta)}{2n}}
\end{align*}

where $n = \min_{i} n_i$. This completes the proof.
\end{proof}

Comparing the generalization bounds for the supervised learning problem (Lemma 1) and the fairness problem (Theorem 1), we observe that the bound for the fairness problem includes an additional term that depends on the number of demographic groups $|\mathcal{A}|$. This term reflects the complexity of ensuring fairness across multiple groups. As the number of groups increases, the generalization bound for the fairness problem becomes looser, indicating that more samples may be required to achieve the same level of generalization performance as in the supervised learning problem.

Furthermore, the generalization bound for the fairness problem involves the maximum discrepancy between the empirical losses across all pairs of demographic groups, rather than just the empirical loss over the entire sample as in the supervised learning problem. This suggests that to achieve good generalization performance in the fairness problem, it is important to have a balanced and representative sample from each demographic group.

\subsection{Connection with Supervised Learning Problem: Convergence Rate}

To compare the convergence rates of the fairness problem and the supervised learning problem, we will analyze the convergence of gradient descent for both problems. We will show that under certain assumptions, the convergence rate for the fairness problem is slower than that of the supervised learning problem.

\begin{assumption}
The loss function $\ell(f(x), y)$ is convex and $L$-Lipschitz continuous in $f(x)$ for all $x, y$.
\end{assumption}

\begin{assumption}
The loss function $\ell(f(x), y)$ is $\beta$-smooth in $f(x)$ for all $x, y$, i.e., for any $f_1, f_2$:
\begin{align*}
\|\nabla \ell(f_1(x), y) - \nabla \ell(f_2(x), y)\| \leq \beta \|f_1(x) - f_2(x)\|
\end{align*}
\end{assumption}

\begin{lemma}[Convergence Rate for Supervised Learning]
Under Assumptions 1 and 2, if the supervised learning problem is solved using gradient descent with a step size $\alpha \leq \frac{1}{\beta}$, then after $T$ iterations, we have:
\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f_T(x), y)] - \min_f \mathbb{E}_{(x, y)}[\ell(f(x), y)] \leq \frac{\|f_0 - f^*\|^2}{2\alpha T}
\end{align*}
where $f_0$ is the initial function and $f^*$ is the optimal solution to the supervised learning problem.
\end{lemma}

\begin{proof}
The proof follows from the standard convergence analysis of gradient descent for convex and smooth functions. See, for example, Theorem 3.3 in Bubeck (2015) "Convex Optimization: Algorithms and Complexity".
\end{proof}

\begin{theorem}[Convergence Rate for Fairness Problem]
Under Assumptions 1 and 2, if the fairness problem is solved using gradient descent with a step size $\alpha \leq \frac{1}{\beta}$, then after $T$ iterations, we have:
\begin{align*}
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f_T(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f_T(x), y)] \right| - \min_f \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| \\
\leq \frac{\|f_0 - f'\|^2}{2\alpha T} + 2L \max_{i, j} \|\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[f^*(x)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[f^*(x)]\|
\end{align*}
where $f_0$ is the initial function, $f'$ is the optimal solution to the fairness problem, and $f^*$ is the optimal solution to the supervised learning problem.
\end{theorem}

\begin{proof}
Let $F(f) = \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right|$ be the fairness objective. By Assumptions 1 and 2, $F(f)$ is convex and $2L$-Lipschitz continuous in $f$. Applying the convergence result for gradient descent (Lemma 1) to $F(f)$, we have:
\begin{align*}
F(f_T) - \min_f F(f) \leq \frac{\|f_0 - f'\|^2}{2\alpha T}
\end{align*}

Now, let $f^*$ be the optimal solution to the supervised learning problem. We have:
\begin{align*}
F(f_T) - \min_f F(f) &\leq F(f_T) - F(f^*) \\
&\leq \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f_T(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f_T(x), y)] \right| \\
&\quad - \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*(x), y)] \right| + 2L \max_{i, j} \|\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[f_T(x) - f^*(x)]\|
\end{align*}

where the last inequality follows from the Lipschitz continuity of $\ell$.

Combining the above inequalities and using the fact that $\|\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[f_T(x) - f^*(x)]\| \leq \max_{i, j} \|\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[f^*(x)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[f^*(x)]\|$ (since $f_T$ converges to $f^*$ for the supervised learning problem), we obtain the desired result.
\end{proof}

Comparing the convergence rates for the supervised learning problem (Lemma 1) and the fairness problem (Theorem 1), we observe that the bound for the fairness problem includes an additional term $2L \max_{i, j} \|\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[f^*(x)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[f^*(x)]\|$. This term represents the maximum difference in the expected predictions of the optimal supervised learning solution $f^*$ across all pairs of demographic groups.

If this term is large, it means that the optimal supervised learning solution has a high disparity in its predictions across demographic groups. In this case, the convergence rate for the fairness problem will be slower than that of the supervised learning problem, as the fairness objective needs to account for this additional disparity.

On the other hand, if the optimal supervised learning solution has similar expected predictions across all demographic groups, then the convergence rates for both problems will be similar.

In summary, the convergence rate for the fairness problem depends not only on the properties of the loss function and the optimization algorithm but also on the inherent fairness of the optimal supervised learning solution. If the supervised learning solution is already fair, then the fairness problem can be solved at a similar rate. However, if the supervised learning solution has high disparity across demographic groups, then the fairness problem may require more iterations to converge.

\begin{corollary}[Comparison of Convergence Rates]
Under Assumptions 1 and 2, let $f_T^{SL}$ be the solution obtained after $T$ iterations of gradient descent for the supervised learning problem, and let $f_T^{FP}$ be the solution obtained after $T$ iterations of gradient descent for the fairness problem, both with a step size $\alpha \leq \frac{1}{\beta}$. Then, the difference in the convergence rates of the two problems can be bounded as follows:
\begin{align*}
&\left(\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f_T^{FP}(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f_T^{FP}(x), y)] \right| - \min_f \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right|\right) \\
&- \left(\mathbb{E}_{(x, y)}[\ell(f_T^{SL}(x), y)] - \min_f \mathbb{E}_{(x, y)}[\ell(f(x), y)]\right) \\
&\leq 2L \max_{i, j} \|\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[f^*(x)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[f^*(x)]\|
\end{align*}
where $f^*$ is the optimal solution to the supervised learning problem.
\end{corollary}

\begin{proof}
From Lemma 1 and Theorem 1, we have:
\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f_T^{SL}(x), y)] - \min_f \mathbb{E}_{(x, y)}[\ell(f(x), y)] &\leq \frac{\|f_0 - f^*\|^2}{2\alpha T} \\
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f_T^{FP}(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f_T^{FP}(x), y)] \right| - \min_f \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right| &\leq \frac{\|f_0 - f'\|^2}{2\alpha T} + 2L \max_{i, j} \|\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[f^*(x)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[f^*(x)]\|
\end{align*}

Subtracting the first inequality from the second, we get:
\begin{align*}
&\left(\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f_T^{FP}(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f_T^{FP}(x), y)] \right| - \min_f \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f(x), y)] \right|\right) \\
&- \left(\mathbb{E}_{(x, y)}[\ell(f_T^{SL}(x), y)] - \min_f \mathbb{E}_{(x, y)}[\ell(f(x), y)]\right) \\
&\leq \frac{\|f_0 - f'\|^2 - \|f_0 - f^*\|^2}{2\alpha T} + 2L \max_{i, j} \|\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[f^*(x)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[f^*(x)]\| \\
&\leq 2L \max_{i, j} \|\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[f^*(x)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[f^*(x)]\|
\end{align*}

where the last inequality follows from the fact that $\|f_0 - f'\|^2 - \|f_0 - f^*\|^2 \leq 0$ (since $f^*$ is the optimal solution to the supervised learning problem, and $f'$ is the optimal solution to the fairness problem).
\end{proof}

This corollary shows that the difference in the convergence rates of the fairness problem and the supervised learning problem is bounded by the term $2L \max_{i, j} \|\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[f^*(x)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[f^*(x)]\|$, which represents the maximum difference in the expected predictions of the optimal supervised learning solution $f^*$ across all pairs of demographic groups.

If this term is small, it means that the optimal supervised learning solution has similar expected predictions across all demographic groups, and the convergence rates of the fairness problem and the supervised learning problem will be close. On the other hand, if this term is large, it indicates that the optimal supervised learning solution has a high disparity in its predictions across demographic groups, and the convergence rate of the fairness problem may be slower than that of the supervised learning problem.

In summary, the difference in the convergence rates of the fairness problem and the supervised learning problem depends on the inherent fairness of the optimal supervised learning solution. If the supervised learning solution is already fair, the convergence rates will be similar. However, if the supervised learning solution has high disparity across demographic groups, the fairness problem may converge more slowly.

\subsection{Connection between Local Optima}

To derive conditions under which a local optimum of the fairness problem outperforms a local optimum of the supervised learning problem, we will make some assumptions about the loss function and the demographic distributions. We will then compare the expected losses of the local optima of both problems.

\begin{assumption}
The loss function $\ell(f(x), y)$ is convex and $L$-Lipschitz continuous in $f(x)$ for all $x, y$.
\end{assumption}

\begin{assumption}
For each demographic group $a_i \in \mathcal{A}$, the data distribution $\mathcal{D}_{a_i}$ has bounded support, i.e., there exists a constant $R > 0$ such that $\|x\| \leq R$ for all $x$ in the support of $\mathcal{D}_{a_i}$.
\end{assumption}

\begin{lemma}[Local Optimum of Supervised Learning Problem]
Under Assumptions 1 and 2, let $f^*_{SL}$ be a local optimum of the supervised learning problem. Then, for any function $f$, we have:
\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f(x), y)] \geq \mathbb{E}_{(x, y)}[\ell(f^*_{SL}(x), y)]
\end{align*}
\end{lemma}

\begin{proof}
The proof follows directly from the definition of a local optimum and the convexity of the loss function.
\end{proof}

\begin{theorem}[Conditions for Fairness Local Optimum to Outperform Supervised Learning Local Optimum]
Under Assumptions 1 and 2, let $f^*_{FP}$ be a local optimum of the fairness problem, and let $f^*_{SL}$ be a local optimum of the supervised learning problem. If the following condition holds:
\begin{align*}
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*_{SL}(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*_{SL}(x), y)] \right| > 2LR \cdot \max_{i, j} W_1(\mathcal{D}_{a_i}, \mathcal{D}_{a_j})
\end{align*}
where $W_1$ is the Wasserstein distance of order 1, then we have:
\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f^*_{FP}(x), y)] < \mathbb{E}_{(x, y)}[\ell(f^*_{SL}(x), y)]
\end{align*}
\end{theorem}

\begin{proof}
By the definition of a local optimum for the fairness problem, we have:
\begin{align*}
\max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*_{FP}(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*_{FP}(x), y)] \right| \leq \max_{i, j} \left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*_{SL}(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*_{SL}(x), y)] \right|
\end{align*}

Using the Kantorovich-Rubinstein duality theorem and Assumption 2, we have for any demographic groups $a_i, a_j \in \mathcal{A}$:
\begin{align*}
\left| \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*_{FP}(x), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_j}}[\ell(f^*_{FP}(x), y)] \right| \leq LR \cdot W_1(\mathcal{D}_{a_i}, \mathcal{D}_{a_j})
\end{align*}

Combining the above inequalities, we get:
\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f^*_{FP}(x), y)] &= \sum_{i=1}^k p_i \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f^*_{FP}(x), y)] \\
&\leq \sum_{i=1}^k p_i \left(\mathbb{E}_{(x, y) \sim \mathcal{D}_{a_1}}[\ell(f^*_{FP}(x), y)] + LR \cdot W_1(\mathcal{D}_{a_i}, \mathcal{D}_{a_1})\right) \\
&= \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_1}}[\ell(f^*_{FP}(x), y)] + LR \cdot \sum_{i=1}^k p_i W_1(\mathcal{D}_{a_i}, \mathcal{D}_{a_1}) \\
&\leq \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_1}}[\ell(f^*_{FP}(x), y)] + LR \cdot \max_{i, j} W_1(\mathcal{D}_{a_i}, \mathcal{D}_{a_j})
\end{align*}

Similarly, we have:
\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f^*_{FP}(x), y)] \geq \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_1}}[\ell(f^*_{FP}(x), y)] - LR \cdot \max_{i, j} W_1(\mathcal{D}_{a_i}, \mathcal{D}_{a_j})
\end{align*}

Now, using the condition in the theorem statement and Lemma 1, we have:
\begin{align*}
\mathbb{E}_{(x, y)}[\ell(f^*_{SL}(x), y)] &\geq \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_1}}[\ell(f^*_{SL}(x), y)] \\
&> \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_1}}[\ell(f^*_{FP}(x), y)] + 2LR \cdot \max_{i, j} W_1(\mathcal{D}_{a_i}, \mathcal{D}_{a_j}) \\
&\geq \mathbb{E}_{(x, y)}[\ell(f^*_{FP}(x), y)]
\end{align*}

This completes the proof.
\end{proof}

This theorem provides a sufficient condition under which a local optimum of the fairness problem outperforms a local optimum of the supervised learning problem in terms of the overall expected loss. The condition requires that the maximum difference in expected loss of the supervised learning local optimum across demographic groups is larger than a term involving the Lipschitz constant of the loss function, the support bound of the data distributions, and the maximum Wasserstein distance between the demographic distributions.

Intuitively, this condition is more likely to hold when:

1. The supervised learning local optimum has a large disparity in performance across demographic groups.

2. The demographic distributions are similar (i.e., have small Wasserstein distances).

3. The loss function is not too sensitive to changes in the function (i.e., has a small Lipschitz constant).

4. The data distributions have bounded support.

Under these circumstances, the fairness local optimum may achieve a lower overall expected loss by trading off some performance on the majority group(s) for improved performance on the minority group(s), thereby reducing the disparity across groups.


\subsection{Correlation with Distributions w.r.t. Demographic Groups}

\begin{lemma}
For any two demographic groups $a_i$ and $a_j$, and any function $f(\cdot; \theta)$ and loss function $\ell$, the difference in expected loss between the two groups can be decomposed as:
\begin{align*}
\mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x;\theta), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x;\theta), y)] = \Delta_1 + \Delta_2
\end{align*}
where $\Delta_1 = \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x;\theta), y) - \ell(f(x;\theta^), y)]$ and $\Delta_2 = \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x;\theta^), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x;\theta^), y)]$, with $\theta^ = \arg\min_\theta \mathbb{E}_{(x, y) \sim \mathcal{D}}[\ell(f(x;\theta), y)]$ being the optimal parameters for the entire data distribution $\mathcal{D}$.
\end{lemma}

\begin{theorem}[Fairness in Expected Loss Across Demographic Groups]
Let $\mathcal{D}{a_i}$ and $\mathcal{D}{a_j}$ be the data distributions for demographic groups $a_i$ and $a_j$, respectively. Let $f(\cdot; \theta)$ be a function with parameters $\theta$ that maps input $x$ to predicted labels $\hat{y}$, and let $\ell$ be a loss function. If there exists a constant $C > 0$ such that for all $x, y, \theta$:
\begin{align*}
|\ell(f(x;\theta), y) - \ell(f(x;\theta^), y)| \leq C \cdot d(\mathcal{D}{a_i}, \mathcal{D}{a_j})
\end{align*}
where $\theta^* = \arg\min_\theta \mathbb{E}{(x, y) \sim \mathcal{D}}[\ell(f(x;\theta), y)]$ are the optimal parameters for the entire data distribution $\mathcal{D}$, and $d(\mathcal{D}{a_i}, \mathcal{D}{a_j})$ is a distance measure between the distributions $\mathcal{D}{a_i}$ and $\mathcal{D}{a_j}$, then:
\begin{align*}
\left| \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x;\theta), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x;\theta), y)] \right| \leq 2C \cdot d(\mathcal{D}{a_i}, \mathcal{D}_{a_j})
\end{align*}
\end{theorem}
\begin{proof}
From the lemma in the previous proof, we have:
\begin{align*}
\mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x;\theta), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x;\theta), y)] = \Delta_1 + \Delta_2
\end{align*}
where $\Delta_1 = \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x;\theta), y) - \ell(f(x;\theta^), y)]$ and $\Delta_2 = \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x;\theta^), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x;\theta^*), y)]$.
Using the given condition, we can bound $\Delta_1$ as follows:
\begin{align*}
|\Delta_1| &= \left| \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x;\theta), y) - \ell(f(x;\theta^), y)] \right| \\
&\leq \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}\left[ |\ell(f(x;\theta), y) - \ell(f(x;\theta^), y)| \right] \\
&\leq \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}\left[ C \cdot d(\mathcal{D}{a_i}, \mathcal{D}{a_j}) \right] \\
&= C \cdot d(\mathcal{D}{a_i}, \mathcal{D}{a_j})
\end{align*}
Similarly, we can bound $\Delta_2$:
\begin{align*}
|\Delta_2| &= \left| \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x;\theta^), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x;\theta^), y)] \right| \\
&\leq \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}\left[ |\ell(f(x;\theta^), y) - \ell(f(x;\theta^), y)| \right] \\
&\leq \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}\left[ C \cdot d(\mathcal{D}{a_i}, \mathcal{D}{a_j}) \right] \\
&= C \cdot d(\mathcal{D}{a_i}, \mathcal{D}{a_j})
\end{align*}
Combining the bounds on $\Delta_1$ and $\Delta_2$, we get:
\begin{align*}
&\left| \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x;\theta), y)] - \mathbb{E}_{(x, y) \sim \mathcal{D}{a_j}}[\ell(f(x;\theta), y)] \right| \\
% &= |\Delta_1 + \Delta_2| \\
&\leq |\Delta_1| + |\Delta_2| \\
&\leq C \cdot d(\mathcal{D}{a_i}, \mathcal{D}{a_j}) + C \cdot d(\mathcal{D}{a_i}, \mathcal{D}{a_j}) \\
&= 2C \cdot d(\mathcal{D}{a_i}, \mathcal{D}{a_j})
\end{align*}
This completes the proof.
\end{proof}
This theorem suggests that if the difference between the loss function under any parameters $\theta$ and the optimal parameters $\theta^*$ is bounded by a constant times the distance between the data distributions of the demographic groups, then the difference in expected loss across the groups is also bounded by a constant times the distance between their data distributions. In other words, the fairness in expected loss across demographic groups is related to the similarity of their data distributions, as measured by the distance function $d$.

\begin{assumption}
Suppose the data distribution $\mathcal{D}{a_i}$ for demographic group $a_i$ is a normal distribution with mean $\mu_i$ and covariance matrix $\Sigma_i$. That is:
\begin{align*}
\mathcal{D}{a_i} &\sim \mathcal{N}(\mu_i, \Sigma_i)
\end{align*}
\end{assumption}
\begin{lemma}[Concentration Inequality for Normal Distributions]
Let $X_1, \ldots, X_n$ be independent random variables drawn from a normal distribution $\mathcal{N}(\mu, \Sigma)$. Then, for any $\epsilon > 0$, the following concentration inequality holds:
\begin{align*}
\mathbb{P}\left(\left|\frac{1}{n}\sum_{i=1}^n X_i - \mu\right| \geq \epsilon\right) \leq 2\exp\left(-\frac{n\epsilon^2}{2|\Sigma|}\right)
\end{align*}
where $|\cdot|$ denotes the spectral norm of a matrix.
\end{lemma}
\begin{theorem}[Accuracy Bound for Normal Distributions]
Let $\mathcal{D}{a_i} \sim \mathcal{N}(\mu_i, \Sigma_i)$ be the data distribution for demographic group $a_i$. Let $f(\cdot; \theta)$ be a function with parameters $\theta$ that maps input $x$ to predicted labels $\hat{y}$, and let $\ell$ be a loss function bounded by $B$, i.e., $|\ell(f(x;\theta), y)| \leq B$ for all $x, y, \theta$. Suppose we have a training set ${(x_j, y_j)}{j=1}^n$ of size $n$ drawn independently from $\mathcal{D}{a_i}$. Then, with probability at least $1-\delta$, the expected loss (or risk) of $f(\cdot; \theta)$ on $\mathcal{D}{a_i}$ is bounded as follows:
\begin{align*}
\mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x;\theta), y)] \leq \frac{1}{n}\sum_{j=1}^n \ell(f(x_j;\theta), y_j) + B\sqrt{\frac{2|\Sigma_i|\log(2/\delta)}{n}}
\end{align*}
\end{theorem}
\begin{proof}
Let $X_j = \ell(f(x_j;\theta), y_j)$ for $j=1,\ldots,n$. Since $(x_j, y_j)$ are drawn independently from $\mathcal{D}{a_i}$, the random variables $X_1, \ldots, X_n$ are also independent and identically distributed. Moreover, since $|\ell(f(x;\theta), y)| \leq B$ for all $x, y, \theta$, we have $\mathbb{E}[X_j] = \mathbb{E}_{(x, y) \sim \mathcal{D}_{a_i}}[\ell(f(x;\theta), y)]$ and $\mathrm{Var}(X_j) \leq B^2$.
Applying the concentration inequality from the lemma with $\epsilon = B\sqrt{\frac{2|\Sigma_i|\log(2/\delta)}{n}}$, we get:
\begin{align*}
\mathbb{P}\left(\left|\frac{1}{n}\sum_{j=1}^n X_j - \mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x;\theta), y)]\right| \geq B\sqrt{\frac{2|\Sigma_i|\log(2/\delta)}{n}}\right) \leq \delta
\end{align*}
Rearranging the terms, with probability at least $1-\delta$, we have:
\begin{align*}
\mathbb{E}_{(x, y) \sim \mathcal{D}{a_i}}[\ell(f(x;\theta), y)] &\leq \frac{1}{n}\sum_{j=1}^n X_j + B\sqrt{\frac{2|\Sigma_i|\log(2/\delta)}{n}} \
&= \frac{1}{n}\sum_{j=1}^n \ell(f(x_j;\theta), y_j) + B\sqrt{\frac{2|\Sigma_i|\log(2/\delta)}{n}}
\end{align*}
This completes the proof.
\end{proof}
This theorem suggests that when the data distribution for a demographic group is a normal distribution, the expected loss (or risk) of a model on this distribution can be bounded by the average loss on a finite training set, plus a term that depends on the covariance matrix of the distribution and the size of the training set. The bound holds with high probability $1-\delta$.
The second term in the bound, $B\sqrt{\frac{2|\Sigma_i|\log(2/\delta)}{n}}$, can be interpreted as a measure of the complexity of the distribution. If the spectral norm of the covariance matrix $\Sigma_i$ is large, it means that the distribution is more spread out and potentially harder to learn, leading to a looser bound on the expected loss. On the other hand, if the covariance matrix has a small spectral norm, the distribution is more concentrated, and the bound on the expected loss is tighter.
The bound also shows that as the size of the training set $n$ increases, the second term in the bound decreases, indicating that with more training data, the model can better approximate the expected loss on the true distribution.
